Projecting basis functions with tensor networks for Gaussian process regression

This paper presents a method for approximate Gaussian process (GP) regression with tensor networks (TNs). A parametric approximation of a GP uses a linear combination of basis functions, where the accuracy of the approximation depends on the total number of basis functions $M$. We develop an approach that allows us to use an exponential amount of basis functions without the corresponding exponential computational complexity. The key idea to enable this is using low-rank TNs. We first find a suitable low-dimensional subspace from the data, described by a low-rank TN. In this low-dimensional subspace, we then infer the weights of our model by solving a Bayesian inference problem. Finally, we project the resulting weights back to the original space to make GP predictions. The benefit of our approach comes from the projection to a smaller subspace: It modifies the shape of the basis functions in a way that it sees fit based on the given data, and it allows for efficient computations in the smaller subspace. In an experiment with an 18-dimensional benchmark data set, we show the applicability of our method to an inverse dynamics problem.

==> 0_reviews.tex <==
# review 1
Notation
- The notation sigman for the variance of epsilonn is a
bit misleading, since the index n is used for the
individual data element, but sigman is the same for all
n (it has a uniform value). Perhaps sigmaepsilon would
be better.
[my comment]
I changed this to sigmay

- Why the observations x are in boldface and those of y
aren't?
[my comment]
x is a vector and y is a scalar.

# review 2
To my knowledge, only few works exist that use
tensor networks in the context of Gaussian processes. To
improve your contribution, you may consider presenting an
overview of how your work relates to other contributions that
use TNs for GPs. For example, these works may be
interesting:
- P. Izmailov: Scalable Gaussian Processes with Billions of
Inducing Inputs via Tensor Train Decomposition
- M. Kirstein: Tensor-Train Kernel Learning for Gaussian
Processes
- K. Konstantinidis: Kernel Learning with Tensor Networks

[my comment]
The proposed work is related, but not relevant to this paper, since to be best of the author's knowledge, TNs are used in a different way.

# review 3
The manuscript is well-written. I do not fully understand
how much of an advance this method is over the current SOTA
in scalable GPs for practical (control) problems. The
numerical section is not strong enough for a reader to
understand the benefits of the paper.

1. There is work on kernel interpolation and deep kernel
networks for scalability of GPs, neither of which are
discussed in the introduction, or compared against in the
numerical section. The KISS-GP (kernel interpolation) idea
is especially relevant; c.f.

[a] https://arxiv.org/abs/1503.01057 (KISS-GP)
[b] https://arxiv.org/abs/1511.02222 (Deep kernel learning)
[c] (control-oriented) https://arxiv.org/abs/2211.00077

[my comment]
In the introduction, it is specified, that among the many efforts to scale up GPs, we will be focusing on the reduced-rank method. While e.g. KISS-GP is related work as an alternative method, it is not relevant to this work.

2. Furthermore, the idea of using random Fourier features
for GP approximation is well-known and recently used in
control; a comparison should be made with this very
standard method.

[d] https://www.jmlr.org/papers/volume18/16-579/16-579.pdf (VFF)
[e] References linked to here:
http://random-walks.org/content/misc/rff/rff.html#id5 (page that explains random Fourier features)
[f] (control-oriented) DOI:10.1016/j.automatica.2021.109613

[my comment]
In the experiment, we compare to the reduced-rank approach which uses regular Fourier features.

3. Are there existing uniform convergence guarantees or
decay rates that could support how many basis functions are
needed for a given $\epsilon$ accuracy?

[my comment]
There are no guarantees for a given epsilon but the paper by Solin and Sarkka shows that the kernel function approximation converges to the true kernel for an infinite number of basis functions.

5. There are no ablation studies. How does the performance
change with no. of basis functions? Computation times with
increasing/decreasing datasets, etc. Since the paper is
mostly algorithmic, a few more experiments and quantitative
comparisons would have made the contributions more
tangible.

[my comment]
We added an large-scale experiment.

7. The fundamental advance of this paper does not
immediately apply to control/estimation theory. There are
control-oriented issues where specific improvements to GPs
can help, e.g. dimensions in control problems may be small
compared to audio/video/image processing but the number of
data points in the sequence may be larger. Another example
is that GPs are used for predictive modeling for MPC, but
the example here does not showcase that.

 [my comment]
 In the introduction, we made clear what the link to control is and in the inverse dynamics experiment, we apply our method to a control-related problem.




==> 1_Introduction_old.tex <==
\section{Introduction}

We will alleviate the prohibitive training cost of GPs exploiting the attractive properties of TN. In particular, we integrate TN into an existing approach by \cite{HilbertGP} that uses basis functions to approximate the kernel function. By doing so, we can apply the alternating linear scheme in a Bayesian framework and reduce the computational cost from $\mathcal{O}(NM^2)$ to $\mathcal{O}(M_dR^2)$ for inference, where $N$ is the number of data points, $M_d$ is the number of basis functions per a dimension, and $R$ is a parameter, called rank, that characterized a TN. The obtained accuracy is competitive with the compared method. Mention hyperparameter training.


Even though the computational complexity of the reduced-rank approach is significantly reduced compared to $\mathcal{O}(N^3)$, the matrix $\bphi\in\mathbb{R}^{N\times M}$ needs to be explicitly built. For a large number of dimensions and/or a high number of required basis functions, this matrix can be become very large.

Approximating kernel functions for high-dimensional problems, requires a number of basis functions $M$ that grow exponentially with the number of input dimensions $D$.
Thus, computing the pseudo-inverse of $\bphi\in\mathbb{R}^{N\times M}$ to solve the linear system in \eqref{eq:model_w} becomes prohibitively expensive.

To reduce the cost of GP predictions, we present a method involving a TT decomposition that avoids the explicit construction and computation of the pseudo-inverse of $\bphi\in\mathbb{R}^{N\times M}$. 
In this context, the number of basis functions are chosen per dimension and each dimension is treated separately, such that the total number of basis functions of $M~=~\prod_{d=1}^D M_d$ does not cause a computational bottleneck.


\begin{itemize}
    \item hilbert-gp chooses function based on leading eigenvalues, based on its ev spectrum. We compare this to avoiding a pre-selection and weighting the basis functions instead. Also: how are dominant eigenfunctions chosen when dimensionality is very high? are all eigenvalues computed? that would mean a lot of sorting
\end{itemize}





==> 3_Methods_old.tex <==
\clearpage
\section{Methods - old}



















Given the approximation in \eqref{eq:truncseries}, the kernel matrices involved in GP regression can be approximately written as
\begin{equation}
    \begin{aligned}
    \K\approx\bphi\boldsymbol\Lambda\bphi^\top,\; \kk_*\approx \boldsymbol\phi_*\boldsymbol\Lambda\bphi^\top,\; k_{**}\approx \boldsymbol\phi_*\boldsymbol\Lambda\boldsymbol\phi_*^\top
    \end{aligned}
    \label{eq:kernapprox}
\end{equation}
 where $\bphi\in\mathbb{R}^{N\times M}$ and $\boldsymbol\phi_*\in\mathbb{R}^{1\times M}$ contain the eigenvectors and $\boldsymbol\Lambda\in\mathbb{R}^{M\times M}$ contains the eigenvalues on the diagonal. 
Prediction equations for unseen inputs for the reduced-rank GP approach are given by 
\begin{equation}
    \begin{aligned}
    \mathbb{E}(f_*) &\approx \boldsymbol\phi_*(\bphi^\top\bphi+\sigma_n^2\boldsymbol\Lambda^{-1})^{-1}\bphi^\top\y\\
    \mathbb{V}(f_*) &\approx \sigma_n^2 \boldsymbol\phi_*(\bphi^\top\bphi+\sigma_n^2\boldsymbol\Lambda^{-1})^{-1}\boldsymbol\phi_*^\top.
    \end{aligned}
    \label{eq:pred_hilbertgp}
\end{equation}


==> 4_Experiments_old.tex <==
\clearpage
\section{Numerical Experiments}
In this section, we present the results of two numerical experiments. All experiments were performed on Dell laptop [specs].

do 3D example and compare to Hilbert GP and show that for full rank it is the same, because same number of free parameters

rank is additional hyperparameter, add discussion about how it can be chosen and how the choice effects the results. Try sampling from the posterior with different kinds of approximations



\subsection{Large-scale example}
To assess the efficiency of the proposed algorithm, we test it on a large-scale 3D data set. The measurements originate from a motion capture suit that measures the position of 17 sensors as well as the magnetic field strength, among other things. We are interested in building a map of a magnetic field in a volume using as many measurements as possible. To test the efficiency, the time the algorithms requires is measured using subsets of increasing size.

\subsection{Prediction accuracy for synthetic data with optimized hyperparameters}
In our third experiment, we make a similar analysis as in the previous experiment. 
The difference is, however, that we do not use the hyperparameters with which we generated the data, but we use optimized ones. 
We take four data sets created from the model \eqref{eq:paramm} for the ranks given in Table \ref{tab:expparams}, and perform hyperparameter optimization with the full GP model on each data set with the Julia package by \cite{JuliaGPpackage}. 
Next, we subdivide the data into 10 different groups of 4000 data points for training and use the remaining data points for validation.

Figure \ref{fig:reerr_hyp} shows that the full GP performs approximately the same on all data sets.
The reduced-rank and Algorithm~\ref{alg:algi} approach perform similarly to the experiment when hyperparameters were not optimized. 

Lastly, we look at the mean standardized log loss (MSLL), defined as 
\begin{equation}
\begin{aligned}
    \mathrm{MSLL} &= \\\frac{1}{2N_*}&\sum_{n_*=1}^{N_*}\left( \frac{([\f_\text{val}]_{n_*}-[\mathbb{E}(\f_*)]_{n_*})^2}{[\mathbb{V}(\f_*)]_{n_*}} + \log 2\pi [\mathbb{V}(\f_*)]_{n_*} \right),
\end{aligned}
\end{equation}
to have a measure for the covariance estimate, where $\f_\text{val}$ are the validation values. 
Figure \ref{fig:MSLL} shows that the MSLL are similar for the full GP and Algorithm \ref{alg:algi}, and that the MSLL is increasing for smaller ranks for the reduced-rank approach. 

\begin{figure}
    \centering
    \input{Figures/rel_err_hyp}
    \caption{Relative error on validation data for data generated from model \eqref{eq:paramm} with varying ranks for optimized hyperparameters. Mean and standard deviation plotted from 10 different parts of the data.}
    \label{fig:reerr_hyp}
\end{figure}


==> Notes.tex <==
\begin{itemize}
    \item \cite[Sec. 2.1.2]{comon2009tensor}. \textcolor{red}{is reference correct?} 
\end{itemize}

==> parking.tex <==
\subsection{things i have tried}
\begin{itemize}
    \item synth data for 2D works (figure \ref{fig:2D_full} and \ref{fig:2D_tt}), certainly is a bit lower for TT approx (script: BayALS\_2D\_experiment)
    \item synth data for 3D or more has numerical issues for the covariance matrix. Also sth weird: inv$\Lambda$ has super large values (because computed from Kronecker product over dimensions) such that first residual always close to 1 (script: BayALS\_experiment)
    \item with orthogonalization no numerical issues but also no good approximation for covariance matrix, not sure if orthogonalization is done correctly for the covariance. Sth to discuss: the prior covariance is dependent on all fixed cores, what is the interpretation of that? Is that ok? (script: BayALS\_experiment)
    \item MALS to compute weights, when dividing the two updated cores of w with SVD, w always want to be full rank... (script: MALS\_krtt\_test, function: MALS\_krtt), Why? Is there a mistake?
    \item modified version where Lambda is absorbed into the Phi matrices. Then the prior covariance becomes diagonal.. does that make sense? tried it for normal Hilbert-GP and gives the same result as normal Hilbert-GP (script BayALS\_mod\_experiment). Also with TTs acceptable results. no SPD problems for cova matrix
    \item finding an approx of covariance matrix for precipitation data set, approx not good.. so computing predictions with TTs makes no sense yet (script: BayALS\_precip)
    \item We split the basis functions over dimensions, so obviously CoD, but both inducing input and basis function papers report that they dont need too many ip or bs, so how are they chosen?
    \item hyperparam opt: phi*phiT needs to be computed. Only once but that is quiet expensive. Is there a better way?
    \item Motion capture suit data: 3D magnetic field data, where is the limit for N? what poses the limit?
\end{itemize}

TO DOS
\begin{itemize}
    \item notation: subscripts ff, * ect, element of matrix/tensor
    \item try cross validation for hyper param opt or compute ALS for product of invZ*Phi
\end{itemize}

In this context, it is considered an approximation of the kernel matrix that is mathematically equivalent to \eqref{eq:kernapprox}, where we redefine $\bphi$ and $\boldsymbol\phi_*$ as a scaled version of themselves, given by
\begin{equation}
    \begin{aligned}
\bphi&:=\bphi\sqrt{\boldsymbol\Lambda},\;\; \boldsymbol\phi_*:=\boldsymbol\phi_*\sqrt{\boldsymbol\Lambda},\;\;\text{where}\;\; \sqrt{\boldsymbol\Lambda}^\top\sqrt{\boldsymbol\Lambda}=\boldsymbol\Lambda,
    \end{aligned}
\end{equation}
and leading to the approximations
\begin{equation}
    \begin{aligned}
        \K\approx\bphi\bphi^\top\;\;\text{and}\;\; \kk_*\approx\bphi\boldsymbol\phi_*^\top.
        \label{eq:kernapproxhat}
    \end{aligned}
\end{equation}


\subsection{Tensor networks}
A multidimensional array, also called a tensor can be represented by smaller interconnected tensors that form a TN. 
An extensive review about TNs can be found in \cite{Kolda2009}. 
The most notable are the CP decomposition, the Tucker decomposition, and the TT decomposition. 
Without loss of generality, we will focus on the TT decomposition in this paper.

\subsubsection*{Tensor notation}
A $D$-way tensor is a generalization of a vector or a matrix to higher dimensions, where $D$ is referred to as the order of the tensor. We denote tensors by calligraphic, boldface, capital letters (e.g.\ $\At$) and matrices, vectors and scalars by boldface capital (e.g.\ $\mathbf{A}$), boldface lowercase (e.g.\ $\mathbf{a}$) and italic lower case (e.g.\ $a$) letters, respectively.

Furthermore, indices or entries of a tensor or matrix are denoted as a subscript of the tensor or matrix between square brackets e.g.\ $[\At]_{i_1 i_2 i_3}$ and $[\A]_{i_1 i_2}$. 
While indices are denoted by a small letter, the size of the corresponding dimension is denotes by a capital letter, e.g.\ $\At \in \mathbb{R}^{I_1\times I_2 \times \hdots \times I_D}$. In addition, a vector of zeros of size $I$ is denoted by $\boldsymbol0_I$ and the identity matrix of size $I\times I$ is denoted by $\id_I$.

\subsubsection*{Tensor Train decomposition}
The tensor train (TT) decomposition, introduced by \cite{Oseledets2011}, consists of a set of three-way tensors $\At_d\in \mathbb{R}^{R_d\times I_d \times R_{d+1}}$, $d=1,..,D$ called TT-cores, that represent a vector $\aaa\in\mathbb{R}^{I_1I_2\dots I_D}$ transformed into a $D$-way tensor $\At\in\mathbb{R}^{I_1\times I_2\times \hdots\times I_D}$ such that $\aaa$ is the vectorization of $\At$. Element-wise, $[\At]_{i_1i_2\dots i_D}$ can be computed as
\begin{equation*}
\sum_{r_1=1}^{R_1}\sum_{r_2=1}^{R_2} \cdots \sum_{r_{D+1}=1}^{R_{D+1}} \left[\At_1\right]_{r_1i_1r_2}\left[\At_2\right]_{r_2i_2r_3}\cdots\left[\At_D\right]_{r_Di_Dr_{D+1}},
\end{equation*}
where $R_1,\dots,R_{D+1}$ are called the ranks of the TT decomposition and by definition $R_1= R_{D+1}=1$.
Assuming without loss of generality that is it $I_1=I_2=\dots I_D=I$ and $R_2=R_3=\dots R_D=R$, the storage complexity of a TT is $\mathcal{O}(DIR^2)$.
The ranks are essential parameters of a TT as they defines both the accuracy of the approximation, as well as its storage complexity.
Comparing a TT's storage complexity to the one of the vector it represents, namely $\mathcal{O}(I^D)$, two main aspects become evident. 
First, the complexity of the TT is not exponential, but linear in $D$, thus is does not suffer from the curse of dimensionality. 
Second, the complexity of the TT depends quadratically on the rank, thus the ranks need to be small to achieve a great compression potential.
The choice of the ranks is dependent on the application and will be discussed later in this paper.

The suitability of modeling large vectors as a low-rank TN has been shown from a theoretical perspective in \cite{shi2021compressibility} and practical in [Freds Nystrom paper, is there a preprint?].



\subsection{Synthetic 2D example}
To test the algorithm a 2D data set is generated. The $N=400$ inputs are random samples in a square from -1,1 in both dimensions and the output data is drawn from a GP with a squared exponential kernel and hyperparameters $((\ell_1^2,\ell_2^2),\sigma_f^2,\sigma_n^2)=[[0.05,0.05],1.0,0.01]$. In the experiment the same hyperparameters are used to describe the model. In both dimensions 30 basis functions are chosen.

Figure \ref{fig:2D_full_long} and \ref{fig:2D_full_short} show the predictions for the full GP together with the training locations. The black lines indicate fixed locations along the first dimension to plot the predictions of the approximation. The approximation is shown in Figures \ref{fig:slice1}-\ref{fig:slice2} and \ref{fig:slice1_long}-\ref{fig:slice2_long} for the middle rank $R=1,5,15$. The figures clearly show that the rank-1 approximation is not producing good results for neither the mean nor the covariance. For $R=5,10$, the mean is much better, the results are overconfident for $R=5$ and under confident for $R=10$.

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/2d_synthdata_fullGP_with_locatiions_short.PNG}
    \caption{Full GP, transparency indicates uncertainty, dots are measurements, black lines are slices where prediction values are plotted together with uncertainty bounds in Figures \ref{fig:slice1}-\ref{fig:slice2}.}
    \label{fig:2D_full_short}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/2d_synthdata_fullGP_with_locatiions_long.PNG}
    \caption{Full GP, transparency indicates uncertainty, dots are measurements, black lines are slices where prediction values are plotted together with uncertainty bounds in Figures \ref{fig:slice1}-\ref{fig:slice2}.}
    \label{fig:2D_full_long}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/slice1.PNG}
    \caption{Predictions along first black line from Figure \ref{fig:2D_full_short} for approximations with different ranks in comparison to full GP.}
    \label{fig:slice1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/slice2.PNG}
    \caption{Predictions along second black line from Figure \ref{fig:2D_full_short} for approximations with different ranks in comparison to full GP.}
    \label{fig:slice2}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/slice1_long.PNG}
    \caption{Predictions along first black line from Figure \ref{fig:2D_full_long} for approximations with different ranks in comparison to full GP.}
    \label{fig:slice1_long}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/slice2_long.PNG}
    \caption{Predictions along second black line from Figure \ref{fig:2D_full_long} for approximations with different ranks in comparison to full GP.}
    \label{fig:slice2_long}
\end{figure}

\subsubsection{Theoretical observations}
When $R$ is chosen to be equal to $M_d$, then the mean of the posterior $\w$ is the same as the mean computed with Hilbert-GP. This is not the case for the covariance matrix. For the covariance matrix, if the TT is chosen to be full rank, the covariance matrices of the single TT-cores may loose positive definitness. 

Note that the matrix $\bphi$ only depends on the input data and $\boldsymbol\Lambda$ only depends on the hyperparameters of the GP model.


We can sample from different models
\begin{equation}
    \begin{aligned}
    \y &= \operatorname{chol}(\K)\aaa, \aaa\sim \mathcal{N}(0,\id)\\
    \y &= \bphi\w, \w\sim \mathcal{N}(0,\boldsymbol\Lambda)\\
    \y &= \bphi\w, \w\sim \mathcal{N}(0,\id) \text{(still GP or not?)}\\
    \y &= \bphi\Wd\w^{(d)}, \w^{(d)}\sim \mathcal{N}(0,\Wd)
    \end{aligned}
\end{equation}
In the first line, we can impose a small length scale such that we need high frequencies. hilbert-GP still performs well though.
In the second line we also use a length scale, so not all basis functions are weighted in a similar way.
In the third line, we consider a function where the high frequency components are weighted in the same way as the low frequency components. Prior on w is still Gaussian, but can this still be a GP? In the ladder case, we cannot impose any length scale.

\subsection{Tensor completion with basis function budget}
In this experiment, we will investigate in a tensor completion setting how our method compares to the reduced-rank approach when imposing a constraint on the number of basis functions, i.e. a basis function budget.

The tensor that has missing entries is a $512\times512$ pixel colored image as shown in Figure ....
When factorizing the row and column dimension, the image is reshaped into a 7-way tensor $\mathbfcal{I}\in\mathbb{R}^{8\times8\times8\times8\times8\times8\times3}$, where the last dimension correspond to the rgb values.
The missing entries are 90\% of the pixels, chosen at random.

As error measures, we consider the relative error, the standardized mean squared error (SMSE) and the mean standardized log loss (MSLL), defines as
\begin{equation}
    \begin{aligned}
    \mathrm{RE} &= \frac{\f_\mathrm{validation}-\mathbb{E}(\f_*)}{\f_\mathrm{validation}}\\
    \mathrm{SMSE} & = \sum_{n_*=1}^{N_*} \frac{[\f_\mathrm{validation}]_{n_*}-[\mathbb{E}(\f_*)]_{n_*}}{\mathbb{V}(\f_\mathrm{validation})} \\
    \mathrm{MSLL} & = \frac{1}{2N_*}\sum_{n_*}^{N_*}\left( \frac{[\f_\mathrm{validation}]_{n_*}-[\mathbb{E}(\f_*)]_{n_*}}{[\mathbb{V}(\f_*)]_{n_*}} + \log 2\pi [\mathbb{V}(\f_*)]_{n_*} \right)
    \end{aligned}
\end{equation}


In \cite[Sec. 4.3]{HilbertGP} it is argued, however, that in higher dimensions, the required basis functions do not exponentially increase in $D$.

\textcolor{red}{improve this:}
Note that the overall weight vector $\W_{\setminus2}\w^{(2)}$ in model \eqref{eq:modelexp} is not sampled according to the squared exponential kernel function, which requires $\w\sim \mathcal{N}(\boldsymbol0,\id_N)$ as given in \eqref{eq:weightedmodel}.
Generally it is, however,
\begin{equation}
    \begin{aligned}
    \w^{(d)}&\sim\mathcal{N}( \boldsymbol0,\id_{R_dM_dR_{d+1}})\\
    \Wd\w^{(d)}&\sim\mathcal{N}( \boldsymbol0,\Wd\Wd^\top)\\
    \Wd\Wd^\top & \neq \id_N.
    \end{aligned}
\end{equation}
In the limit of $\Wd$ being square, corresponding to a full-rank TT, the samples are distributed according to the squared exponential.

Another motivation to use TN is that they enable efficient algorithms which in turn are more sustainable and can be called Green AI, as argued in \cite{memmel2022towards}.

The basis functions that best describe the kernel function are not chosen based on the leading eigenvalues, but by projecting the basis functions into a smaller subspace.
In this way, higher-frequent basis functions are not discarded, when the computational budget does not allow for a high number of basis function to approximate the kernel function.


% Recommended preamble:
\begin{tikzpicture}
\begin{axis}[xmajorgrids, ymajorgrids, xlabel={TT-ranks}, ylabel={RMSE}, xtick={1,2,3,4}, xticklabels={1,5,10,20}, style = {very thick}]
    \addplot[color={red}, mark={x}, error bars/y dir=both, error bars/y explicit]
        coordinates {
            (1,0.8548488000000003) +- (0,0.15855295627560317)
            (2,0.3905046) +- (0,0.02058131212856297)
            (3,0.31306750000000005) +- (0,0.015708690427417696)
            (4,0.27919499999999997) +- (0,0.009568455895400384)
        }
        ;
    \addplot[color={blue}, mark={x}, error bars/y dir=both, error bars/y explicit]
        coordinates {
            (1,0.9786296) +- (0,0.04006252166080191)
            (2,0.6403738000000001) +- (0,0.037763301211626056)
            (3,0.39609749999999994) +- (0,0.029091398615207355)
            (4,0.27780689999999997) +- (0,0.009028143853159042)
        }
        ;
    \addplot[color={green}, mark={x}, error bars/y dir=both, error bars/y explicit]
        coordinates {
            (1,0.03444092000000001) +- (0,0.0031263041370495825)
            (2,0.120855) +- (0,0.0075953653851104095)
            (3,0.2461954) +- (0,0.016573944941785386)
            (4,0.27780689999999997) +- (0,0.009028143853159042)
        }
        ;
    \legend{{Full GP},{Hilbert-GP},{Algorithm \ref{alg:algi}}}
\end{axis}
\end{tikzpicture}
